Understanding the Sparse Vector Technique for Differential Privacy

The Sparse Vector Technique (SVT) is a fundamental technique for satisfying differential privacy and has the unique quality that one can output some query answers without apparently paying any privacy cost. SVT has been used in both the interactive setting, where one tries to answer a sequence of queries that are not known ahead of the time, and in the non-interactive setting, where all queries are known. Because of the potential savings on privacy budget, many variants for SVT have been proposed and employed in privacy-preserving data mining and publishing. However, most variants of SVT are actually not private. In this paper, we analyze these errors and identify the misunderstandings that likely contribute to them. We also propose a new version of SVT that provides better utility, and introduce an effective technique to improve the performance of SVT. These enhancements can be applied to improve utility in the interactive setting. Through both analytical and experimental comparisons, we show that, in the non-interactive setting (but not the interactive setting), the SVT technique is unnecessary, as it can be replaced by the Exponential Mechanism (EM) with better accuracy.

==> figures/comparison/TOPK_SUM_RATIO_0.1_AOL.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(2340.00,1411.20)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,704){\makebox(0,0)[r]{\strut{}0.0}}%
      \put(946,748){\makebox(0,0)[r]{\strut{}0.1}}%
      \put(946,793){\makebox(0,0)[r]{\strut{}0.2}}%
      \put(946,837){\makebox(0,0)[r]{\strut{}0.3}}%
      \put(946,881){\makebox(0,0)[r]{\strut{}0.4}}%
      \put(946,926){\makebox(0,0)[r]{\strut{}0.5}}%
      \put(946,970){\makebox(0,0)[r]{\strut{}0.6}}%
      \put(946,1014){\makebox(0,0)[r]{\strut{}0.7}}%
      \put(946,1058){\makebox(0,0)[r]{\strut{}0.8}}%
      \put(946,1103){\makebox(0,0)[r]{\strut{}0.9}}%
      \put(946,1147){\makebox(0,0)[r]{\strut{}1.0}}%
      \put(1078,484){\makebox(0,0){\strut{}25}}%
      \put(1157,484){\makebox(0,0){\strut{}50}}%
      \put(1235,484){\makebox(0,0){\strut{}75}}%
      \put(1314,484){\makebox(0,0){\strut{}100}}%
      \put(1393,484){\makebox(0,0){\strut{}125}}%
      \put(1471,484){\makebox(0,0){\strut{}150}}%
      \put(1550,484){\makebox(0,0){\strut{}175}}%
      \put(1628,484){\makebox(0,0){\strut{}200}}%
      \put(1707,484){\makebox(0,0){\strut{}225}}%
      \put(1786,484){\makebox(0,0){\strut{}250}}%
      \put(1864,484){\makebox(0,0){\strut{}275}}%
      \put(1943,484){\makebox(0,0){\strut{}300}}%
      \put(176,925){\rotatebox{-270}{\makebox(0,0){\strut{}SUM RATIO}}}%
      \put(1510,154){\makebox(0,0){\strut{}Top-K}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{TOPK_SUM_RATIO_0.1_AOL}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/comparison/TOPK_SUM_RATIO_0.1_BMS-POS.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(2340.00,1411.20)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,704){\makebox(0,0)[r]{\strut{}0.0}}%
      \put(946,748){\makebox(0,0)[r]{\strut{}0.1}}%
      \put(946,793){\makebox(0,0)[r]{\strut{}0.2}}%
      \put(946,837){\makebox(0,0)[r]{\strut{}0.3}}%
      \put(946,881){\makebox(0,0)[r]{\strut{}0.4}}%
      \put(946,926){\makebox(0,0)[r]{\strut{}0.5}}%
      \put(946,970){\makebox(0,0)[r]{\strut{}0.6}}%
      \put(946,1014){\makebox(0,0)[r]{\strut{}0.7}}%
      \put(946,1058){\makebox(0,0)[r]{\strut{}0.8}}%
      \put(946,1103){\makebox(0,0)[r]{\strut{}0.9}}%
      \put(946,1147){\makebox(0,0)[r]{\strut{}1.0}}%
      \put(1078,484){\makebox(0,0){\strut{}25}}%
      \put(1157,484){\makebox(0,0){\strut{}50}}%
      \put(1235,484){\makebox(0,0){\strut{}75}}%
      \put(1314,484){\makebox(0,0){\strut{}100}}%
      \put(1393,484){\makebox(0,0){\strut{}125}}%
      \put(1471,484){\makebox(0,0){\strut{}150}}%
      \put(1550,484){\makebox(0,0){\strut{}175}}%
      \put(1628,484){\makebox(0,0){\strut{}200}}%
      \put(1707,484){\makebox(0,0){\strut{}225}}%
      \put(1786,484){\makebox(0,0){\strut{}250}}%
      \put(1864,484){\makebox(0,0){\strut{}275}}%
      \put(1943,484){\makebox(0,0){\strut{}300}}%
      \put(176,925){\rotatebox{-270}{\makebox(0,0){\strut{}SUM RATIO}}}%
      \put(1510,154){\makebox(0,0){\strut{}Top-K}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{TOPK_SUM_RATIO_0.1_BMS-POS}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/comparison/TOPK_SUM_RATIO_0.1_kosarak.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(2340.00,1411.20)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,704){\makebox(0,0)[r]{\strut{}0.0}}%
      \put(946,748){\makebox(0,0)[r]{\strut{}0.1}}%
      \put(946,793){\makebox(0,0)[r]{\strut{}0.2}}%
      \put(946,837){\makebox(0,0)[r]{\strut{}0.3}}%
      \put(946,881){\makebox(0,0)[r]{\strut{}0.4}}%
      \put(946,926){\makebox(0,0)[r]{\strut{}0.5}}%
      \put(946,970){\makebox(0,0)[r]{\strut{}0.6}}%
      \put(946,1014){\makebox(0,0)[r]{\strut{}0.7}}%
      \put(946,1058){\makebox(0,0)[r]{\strut{}0.8}}%
      \put(946,1103){\makebox(0,0)[r]{\strut{}0.9}}%
      \put(946,1147){\makebox(0,0)[r]{\strut{}1.0}}%
      \put(1078,484){\makebox(0,0){\strut{}25}}%
      \put(1157,484){\makebox(0,0){\strut{}50}}%
      \put(1235,484){\makebox(0,0){\strut{}75}}%
      \put(1314,484){\makebox(0,0){\strut{}100}}%
      \put(1393,484){\makebox(0,0){\strut{}125}}%
      \put(1471,484){\makebox(0,0){\strut{}150}}%
      \put(1550,484){\makebox(0,0){\strut{}175}}%
      \put(1628,484){\makebox(0,0){\strut{}200}}%
      \put(1707,484){\makebox(0,0){\strut{}225}}%
      \put(1786,484){\makebox(0,0){\strut{}250}}%
      \put(1864,484){\makebox(0,0){\strut{}275}}%
      \put(1943,484){\makebox(0,0){\strut{}300}}%
      \put(176,925){\rotatebox{-270}{\makebox(0,0){\strut{}SUM RATIO}}}%
      \put(1510,154){\makebox(0,0){\strut{}Top-K}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{TOPK_SUM_RATIO_0.1_kosarak}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/comparison/TOPK_SUM_RATIO_0.5_AOL.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(2340.00,1411.20)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,704){\makebox(0,0)[r]{\strut{}0.0}}%
      \put(946,748){\makebox(0,0)[r]{\strut{}0.1}}%
      \put(946,793){\makebox(0,0)[r]{\strut{}0.2}}%
      \put(946,837){\makebox(0,0)[r]{\strut{}0.3}}%
      \put(946,881){\makebox(0,0)[r]{\strut{}0.4}}%
      \put(946,926){\makebox(0,0)[r]{\strut{}0.5}}%
      \put(946,970){\makebox(0,0)[r]{\strut{}0.6}}%
      \put(946,1014){\makebox(0,0)[r]{\strut{}0.7}}%
      \put(946,1058){\makebox(0,0)[r]{\strut{}0.8}}%
      \put(946,1103){\makebox(0,0)[r]{\strut{}0.9}}%
      \put(946,1147){\makebox(0,0)[r]{\strut{}1.0}}%
      \put(1078,484){\makebox(0,0){\strut{}25}}%
      \put(1157,484){\makebox(0,0){\strut{}50}}%
      \put(1235,484){\makebox(0,0){\strut{}75}}%
      \put(1314,484){\makebox(0,0){\strut{}100}}%
      \put(1393,484){\makebox(0,0){\strut{}125}}%
      \put(1471,484){\makebox(0,0){\strut{}150}}%
      \put(1550,484){\makebox(0,0){\strut{}175}}%
      \put(1628,484){\makebox(0,0){\strut{}200}}%
      \put(1707,484){\makebox(0,0){\strut{}225}}%
      \put(1786,484){\makebox(0,0){\strut{}250}}%
      \put(1864,484){\makebox(0,0){\strut{}275}}%
      \put(1943,484){\makebox(0,0){\strut{}300}}%
      \put(176,925){\rotatebox{-270}{\makebox(0,0){\strut{}SUM RATIO}}}%
      \put(1510,154){\makebox(0,0){\strut{}Top-K}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{TOPK_SUM_RATIO_0.5_AOL}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/comparison/TOPK_SUM_RATIO_0.5_BMS-POS.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(2340.00,1411.20)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,704){\makebox(0,0)[r]{\strut{}0.0}}%
      \put(946,748){\makebox(0,0)[r]{\strut{}0.1}}%
      \put(946,793){\makebox(0,0)[r]{\strut{}0.2}}%
      \put(946,837){\makebox(0,0)[r]{\strut{}0.3}}%
      \put(946,881){\makebox(0,0)[r]{\strut{}0.4}}%
      \put(946,926){\makebox(0,0)[r]{\strut{}0.5}}%
      \put(946,970){\makebox(0,0)[r]{\strut{}0.6}}%
      \put(946,1014){\makebox(0,0)[r]{\strut{}0.7}}%
      \put(946,1058){\makebox(0,0)[r]{\strut{}0.8}}%
      \put(946,1103){\makebox(0,0)[r]{\strut{}0.9}}%
      \put(946,1147){\makebox(0,0)[r]{\strut{}1.0}}%
      \put(1078,484){\makebox(0,0){\strut{}25}}%
      \put(1157,484){\makebox(0,0){\strut{}50}}%
      \put(1235,484){\makebox(0,0){\strut{}75}}%
      \put(1314,484){\makebox(0,0){\strut{}100}}%
      \put(1393,484){\makebox(0,0){\strut{}125}}%
      \put(1471,484){\makebox(0,0){\strut{}150}}%
      \put(1550,484){\makebox(0,0){\strut{}175}}%
      \put(1628,484){\makebox(0,0){\strut{}200}}%
      \put(1707,484){\makebox(0,0){\strut{}225}}%
      \put(1786,484){\makebox(0,0){\strut{}250}}%
      \put(1864,484){\makebox(0,0){\strut{}275}}%
      \put(1943,484){\makebox(0,0){\strut{}300}}%
      \put(176,925){\rotatebox{-270}{\makebox(0,0){\strut{}SUM RATIO}}}%
      \put(1510,154){\makebox(0,0){\strut{}Top-K}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{TOPK_SUM_RATIO_0.5_BMS-POS}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/comparison/TOPK_SUM_RATIO_0.5_kosarak.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(2340.00,1411.20)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,704){\makebox(0,0)[r]{\strut{}0.0}}%
      \put(946,748){\makebox(0,0)[r]{\strut{}0.1}}%
      \put(946,793){\makebox(0,0)[r]{\strut{}0.2}}%
      \put(946,837){\makebox(0,0)[r]{\strut{}0.3}}%
      \put(946,881){\makebox(0,0)[r]{\strut{}0.4}}%
      \put(946,926){\makebox(0,0)[r]{\strut{}0.5}}%
      \put(946,970){\makebox(0,0)[r]{\strut{}0.6}}%
      \put(946,1014){\makebox(0,0)[r]{\strut{}0.7}}%
      \put(946,1058){\makebox(0,0)[r]{\strut{}0.8}}%
      \put(946,1103){\makebox(0,0)[r]{\strut{}0.9}}%
      \put(946,1147){\makebox(0,0)[r]{\strut{}1.0}}%
      \put(1078,484){\makebox(0,0){\strut{}25}}%
      \put(1157,484){\makebox(0,0){\strut{}50}}%
      \put(1235,484){\makebox(0,0){\strut{}75}}%
      \put(1314,484){\makebox(0,0){\strut{}100}}%
      \put(1393,484){\makebox(0,0){\strut{}125}}%
      \put(1471,484){\makebox(0,0){\strut{}150}}%
      \put(1550,484){\makebox(0,0){\strut{}175}}%
      \put(1628,484){\makebox(0,0){\strut{}200}}%
      \put(1707,484){\makebox(0,0){\strut{}225}}%
      \put(1786,484){\makebox(0,0){\strut{}250}}%
      \put(1864,484){\makebox(0,0){\strut{}275}}%
      \put(1943,484){\makebox(0,0){\strut{}300}}%
      \put(176,925){\rotatebox{-270}{\makebox(0,0){\strut{}SUM RATIO}}}%
      \put(1510,154){\makebox(0,0){\strut{}Top-K}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{TOPK_SUM_RATIO_0.5_kosarak}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/comparison/TOPK_SUM_RATIO_left.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(2340.00,1411.20)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(814,704){\makebox(0,0)[r]{\strut{}0.0}}%
      \put(814,748){\makebox(0,0)[r]{\strut{}0.1}}%
      \put(814,793){\makebox(0,0)[r]{\strut{}0.2}}%
      \put(814,837){\makebox(0,0)[r]{\strut{}0.3}}%
      \put(814,881){\makebox(0,0)[r]{\strut{}0.4}}%
      \put(814,926){\makebox(0,0)[r]{\strut{}0.5}}%
      \put(814,970){\makebox(0,0)[r]{\strut{}0.6}}%
      \put(814,1014){\makebox(0,0)[r]{\strut{}0.7}}%
      \put(814,1058){\makebox(0,0)[r]{\strut{}0.8}}%
      \put(814,1103){\makebox(0,0)[r]{\strut{}0.9}}%
      \put(946,484){\makebox(0,0){\strut{}25}}%
      \put(1037,484){\makebox(0,0){\strut{}50}}%
      \put(1127,484){\makebox(0,0){\strut{}75}}%
      \put(1218,484){\makebox(0,0){\strut{}100}}%
      \put(1309,484){\makebox(0,0){\strut{}125}}%
      \put(1399,484){\makebox(0,0){\strut{}150}}%
      \put(1490,484){\makebox(0,0){\strut{}175}}%
      \put(1580,484){\makebox(0,0){\strut{}200}}%
      \put(1671,484){\makebox(0,0){\strut{}225}}%
      \put(1762,484){\makebox(0,0){\strut{}250}}%
      \put(1852,484){\makebox(0,0){\strut{}275}}%
      \put(1943,484){\makebox(0,0){\strut{}300}}%
      \put(176,925){\rotatebox{-270}{\makebox(0,0){\strut{}SUM RATIO}}}%
      \put(1444,154){\makebox(0,0){\strut{}Top-K}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1793,1238){\makebox(0,0)[r]{\strut{}SVT-DPBook}}%
      \csname LTb\endcsname%
      \put(1793,1018){\makebox(0,0)[r]{\strut{}SVT-1:1}}%
      \csname LTb\endcsname%
      \put(1793,798){\makebox(0,0)[r]{\strut{}SVT-1:3}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{TOPK_SUM_RATIO_left}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/comparison/TOPK_SUM_RATIO_right.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(2340.00,1411.20)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(814,704){\makebox(0,0)[r]{\strut{}0.0}}%
      \put(814,704){\makebox(0,0)[r]{\strut{}0.1}}%
      \put(814,705){\makebox(0,0)[r]{\strut{}0.2}}%
      \put(814,705){\makebox(0,0)[r]{\strut{}0.3}}%
      \put(814,705){\makebox(0,0)[r]{\strut{}0.4}}%
      \put(814,706){\makebox(0,0)[r]{\strut{}0.5}}%
      \put(814,706){\makebox(0,0)[r]{\strut{}0.6}}%
      \put(814,706){\makebox(0,0)[r]{\strut{}0.7}}%
      \put(814,706){\makebox(0,0)[r]{\strut{}0.8}}%
      \put(814,707){\makebox(0,0)[r]{\strut{}0.9}}%
      \put(946,484){\makebox(0,0){\strut{}25}}%
      \put(1037,484){\makebox(0,0){\strut{}50}}%
      \put(1127,484){\makebox(0,0){\strut{}75}}%
      \put(1218,484){\makebox(0,0){\strut{}100}}%
      \put(1309,484){\makebox(0,0){\strut{}125}}%
      \put(1399,484){\makebox(0,0){\strut{}150}}%
      \put(1490,484){\makebox(0,0){\strut{}175}}%
      \put(1580,484){\makebox(0,0){\strut{}200}}%
      \put(1671,484){\makebox(0,0){\strut{}225}}%
      \put(1762,484){\makebox(0,0){\strut{}250}}%
      \put(1852,484){\makebox(0,0){\strut{}275}}%
      \put(1943,484){\makebox(0,0){\strut{}300}}%
      \put(176,705){\rotatebox{-270}{\makebox(0,0){\strut{}SUM RATIO}}}%
      \put(1444,154){\makebox(0,0){\strut{}Top-K}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4697,1238){\makebox(0,0)[r]{\strut{}SVT-:k^{23}   with errorlines ls 4,}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{TOPK_SUM_RATIO_right}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> table_3.tex <==
\begin{table*}[!ht]
\centering
\small
%\begin{tabular}{|p{.5in}|p{.2in}|p{.55in}|p{.55in}|p{.55in}|p{.55in}|p{.55in}|p{.55in}|p{.55in}|p{.55in}|}\hline
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}\hline
%\multirow{2}{*}{Dataset Privacy Budget} & \multirow{2}{*}{$c$} & \multirow{2}{*}{DPBook} & \multirow{2}{*}{EM} & \multicolumn{4}{|c|}{SVT} & \multicolumn{2}{|c|}{SVT-ReTr} \\\cline{5-10}
%                         &  & & & $1:1$ & $1:3$ & $1:k$  & $1:k^{2/3}$ & $1:1$ & $1:k^{2/3}$ \\\hline

Dataset & \multirow{3}{*}{$c$} & \multicolumn{5}{|c|}{Interactive Setting} & \multicolumn{4}{|c|}{Non-interactive Setting} \\\cline{3-11}
Budget  &  & \multirow{2}{*}{SVT-DPBook}& \multicolumn{4}{|c|}{SVT-S} & \multicolumn{3}{|c|}{SVT-ReTr-$1:c^{2/3}$}  & \multirow{2}{*}{EM} \\\cline{4-10}
                         &  & & $1:1$ & $1:3$ & $1:c$  & $1:c^{2/3}$ & 1D & 2D & 3D \\\cline{1-11}

\multirow{3}{*}{BMS-POS}
& $50$ & $0.072_{0.051}$ &	$0.017_{0.027}$ &	$\mathbf{0.016_{0.025}}$ &	$0.030_{0.040}$ & $0.017_{0.029}$ &	$\mathit{0.001_{0.001}}$ & $0.004_{0.007}$ & $0.017_{0.010}$ &	$\mathit{0.001_{0.001}}$ \\ \cline{2-11}
& $100$ & $0.561_{0.085}$ &	$0.255_{0.078}$ &	$0.096_{0.047}$ &	$0.101_{0.097}$ & $\mathbf{0.063_{0.055}}$ &	$0.010_{0.019}$  &	$\mathit{0.007_{0.003}}$ &	$0.018_{0.011}$ &	 $\mathit{0.007_{0.003}}$\\ \cline{2-11}
& $150$	& $0.669_{0.073}$ &	$0.505_{0.079}$ &	$0.341_{0.080}$ &	$0.289_{0.221}$ & $\mathbf{0.220_{0.083}}$ & $0.049_{0.012}$ &	$\mathit{0.047_{0.007}}$  &	$0.056_{0.013}$ &	$0.048_{0.006}$\\ \cline{2-11}
\multirow{2}{*}{$\epsilon=0.1$}
& $200$	& $0.682_{0.071}$ &	$0.628_{0.069}$ &	$0.562_{0.070}$ &	$0.508_{0.223}$ & $\mathbf{0.478_{0.101}}$ & $0.173_{0.067}$ &	$\mathit{0.091_{0.007}}$  &	$0.092_{0.007}$ &	$0.092_{0.008}$\\ \cline{2-11}
%& $250$	& $0.656_{0.068}$ &	$\mathbf{0.123_{0.007}}$ &	$0.645_{0.068}$ &	$0.598_{0.068}$ &	$0.546_{0.228}$ & $0.556_{0.090}$ & $0.324_{0.059}$ &	$\mathbf{0.221_{0.083}}$\\ \cline{2-10}
& $300$	& $0.621_{0.069}$ &	$0.631_{0.065}$ &	$0.607_{0.064}$ &	$\mathbf{0.535_{0.225}}$ & $0.581_{0.083}$ & $0.224_{0.092}$ &	$\mathit{0.134_{0.008}}$  &	$0.138_{0.007}$ &	$0.141_{0.009}$ \\ \hline\hline
\multirow{3}{*}{Kosarak}
& $50$ & $0.705_{0.142}$ &	$0.047_{0.061}$ &	$0.032_{0.062}$ &	$0.033_{0.063}$ & $\mathbf{0.025_{0.049}}$ &	$0.009_{0.034}$ &	$0.001_{0.001}$  &	$0.005_{0.005}$ &	$\mathit{0.000_{0.000}}$ \\ \cline{2-11}
& $100$ & $0.968_{0.043}$ &	$0.896_{0.080}$ &	$0.640_{0.142}$ &	$\mathbf{0.373_{0.247}}$ & $0.398_{0.144}$ &  $0.103_{0.098}$ & $0.038_{0.009}$ &	$0.040_{0.008}$ &	$\mathit{0.033_{0.005}}$\\ \cline{2-11}
& $150$ & $0.972_{0.037}$ &	$0.956_{0.046}$ &	$0.904_{0.075}$ &	$\mathbf{0.772_{0.208}}$ & $0.818_{0.108}$ & $0.627_{0.134}$ &	$0.276_{0.141}$  &	$0.141_{0.008}$ &	$\mathit{0.139_{0.007}}$ \\ \cline{2-11}
\multirow{2}{*}{$\epsilon=0.1$}
& $200$ & $0.974_{0.037}$ &	$0.967_{0.044}$ &	$0.960_{0.034}$ &	$\mathbf{0.865_{0.177}}$ & $0.942_{0.045}$ & $0.833_{0.107}$ &	$0.656_{0.121}$  &	$0.265_{0.083}$ &	$\mathit{0.219_{0.008}}$ \\ \cline{2-11}
%& $250$ & $0.970_{0.037}$ &	$\mathbf{0.273_{0.008}}$ &	$0.966_{0.038}$ &	$0.958_{0.042}$ &	$0.913_{0.115}$ & $0.945_{0.048}$ & $0.943_{0.051}$ &	$\mathbf{0.883_{0.074}}$\\ \cline{2-10}
& $300$ & $0.971_{0.040}$ &	$0.971_{0.034}$ &	$0.961_{0.039}$ &	$\mathbf{0.945_{0.065}}$ & $0.950_{0.052}$ & $0.902_{0.079}$ &	$0.801_{0.099}$  &	$0.518_{0.130}$ &	$\mathit{0.315_{0.007}}$ \\ \hline\hline
\multirow{3}{*}{AOL}
& $50$ & $0.225_{0.062}$ & $0.016_{0.016}$ &	$0.013_{0.015}$ &	$0.023_{0.023}$ & $\mathbf{0.011_{0.013}}$ & $0.002_{0.005}$ &	$0.003_{0.007}$  & $0.012_{0.011}$ &	$\mathit{0.001_{0.001}}$ \\\cline{2-11}
& $100$ & $0.993_{0.008}$ & $0.739_{0.046}$ &	$0.072_{0.029}$ &	$0.093_{0.093}$ & $\mathbf{0.025_{0.017}}$ & $0.007_{0.006}$ &	$0.007_{0.010}$  & $0.068_{0.034}$ &	$\mathit{0.005_{0.002}}$  \\\cline{2-11}
& $150$ & $0.998_{0.003}$ & $0.986_{0.009}$ &	$0.902_{0.028}$ &	$\mathbf{0.532_{0.215}}$ & $0.587_{0.075}$ & $0.346_{0.082}$ &	$0.178_{0.033}$  & $0.173_{0.014}$ &	$\mathit{0.153_{0.015}}$ \\\cline{2-11}
\multirow{2}{*}{$\epsilon=0.1$}
& $200$ & $0.999_{0.002}$ & $0.996_{0.005}$ &	$0.987_{0.009}$ &	$\mathbf{0.924_{0.090}}$ & $0.955_{0.019}$ & $0.894_{0.031}$ &	$0.787_{0.050}$  & $0.591_{0.073}$ &	$\mathit{0.412_{0.014}}$ \\\cline{2-11}
%& $250$ & $0.999_{0.002}$ & $\mathbf{0.571_{0.013}}$ & $0.998_{0.003}$ &	$0.995_{0.005}$ &	$0.978_{0.043}$ & $0.990_{0.008}$ & $0.996_{0.004}$ &	$\mathbf{0.977_{0.011}}$\\\cline{2-10}
& $300$ & $0.999_{0.002}$ & $0.998_{0.003}$ &	$0.997_{0.003}$ &	$\mathbf{0.986_{0.033}}$ & $0.995_{0.005}$ & $0.990_{0.006}$ &	$0.979_{0.011}$  & $0.955_{0.020}$ &	$\mathit{0.683_{0.014}}$\\\hline\hline
\multirow{3}{*}{Zipf}
& $50$ & $0.957_{0.054}$ & $0.917_{0.076}$ &	$0.832_{0.103}$ &	$0.665_{0.269}$ & $0.711_{0.151}$ &	$0.423_{0.171}$ &	$0.164_{0.118}$  & $0.090_{0.016}$ &	$\mathit{0.082_{0.011}}$ \\\cline{2-11}
& $100$ & $0.969_{0.029}$ & $0.960_{0.053}$ &	$0.955_{0.041}$ &	$0.924_{0.116}$ & $0.944_{0.057}$ & $0.876_{0.083}$ &	$0.750_{0.123}$  & $0.404_{0.118}$ &	$\mathit{0.262_{0.015}}$  \\\cline{2-11}
& $150$ & $0.952_{0.053}$ & $0.952_{0.050}$ &	$0.958_{0.035}$ &	$0.922_{0.094}$ & $0.936_{0.067}$ & $0.896_{0.072}$ &	$0.765_{0.108}$  & $0.468_{0.112}$ &	$\mathit{0.355_{0.017}}$ \\\cline{2-11}
\multirow{2}{*}{$\epsilon=0.1$}
& $200$ & $0.947_{0.049}$ & $0.946_{0.052}$ &	$0.948_{0.038}$ &	$0.898_{0.128}$ & $0.940_{0.047}$ & $0.887_{0.077}$ &	$0.769_{0.105}$  & $0.468_{0.087}$ &	$\mathit{0.412_{0.016}}$ \\\cline{2-11}
%& $250$ & $0.999_{0.002}$ & $\mathbf{0.571_{0.013}}$ & $0.998_{0.003}$ &	$0.995_{0.005}$ &	$0.978_{0.043}$ & $0.990_{0.008}$ & $0.996_{0.004}$ &	$\mathbf{0.977_{0.011}}$\\\cline{2-10}
& $300$ & $0.937_{0.048}$ & $0.939_{0.038}$ &	$0.933_{0.050}$ &	$0.874_{0.113}$ & $0.928_{0.045}$ & $0.867_{0.077}$ &	$0.719_{0.108}$  & $0.485_{0.040}$ &	$\mathit{0.481_{0.020}}$\\\hline\hline
%\end{tabular}
%\caption{Comparison of EM and SVT variants on SUM RATIO, where $\epsilon=0.1$.}\label{tab:method_comp_eps_0.1}
%\end{table*}

%\begin{table*}
%\centering
%\begin{tabular}{|p{.5in}|p{.2in}|p{.55in}|p{.55in}|p{.55in}|p{.55in}|p{.55in}|p{.55in}|p{.55in}|p{.55in}|}\hline
%\multirow{2}{*}{Dataset} & \multirow{2}{*}{$c$} & \multirow{2}{*}{DPBook} & \multirow{2}{*}{EM} & \multicolumn{4}{|c|}{SVT} & \multicolumn{2}{|c|}{SVT-ReTr} \\\cline{5-10}
%                         &  & & & $1:1$ & $1:3$ & $1:k$  & $1:k^{2/3}$ & $1:1$ & $1:k^{2/3}$ \\\hline

\multirow{3}{*}{BMS-POS}
& $50$ & $0.009_{0.011}$ &	$0.008_{0.017}$ &	$0.006_{0.016}$ &	$0.007_{0.017}$ & $\mathbf{0.004_{0.006}}$ &	$\mathit{0.000_{0.002}}$  & $0.002_{0.003}$ & $0.005_{0.005}$ & $\mathit{0.000_{0.000}}$\\ \cline{2-11}
& $100$ & $0.040_{0.034}$ &	$0.011_{0.012}$ &	$0.009_{0.017}$ &	$0.013_{0.021}$ & $\mathbf{0.008_{0.016}}$ &	$\mathit{0.000_{0.001}}$ &	$0.000_{0.001}$ &	$0.003_{0.003}$  & $\mathit{0.000_{0.000}}$\\ \cline{2-11}
& $150$	& $0.113_{0.047}$ &	$0.012_{0.014}$ &	$\mathbf{0.007_{0.005}}$ &	$0.017_{0.019}$ & $0.008_{0.008}$ & $\mathit{0.001_{0.001}}$  &	$0.002_{0.002}$ & $0.014_{0.006}$ &	$\mathit{0.001_{0.000}}$\\ \cline{2-11}
\multirow{2}{*}{$\epsilon=0.5$}
& $200$	& $0.369_{0.067}$ &	$0.123_{0.051}$ &	$0.040_{0.023}$ &	$0.048_{0.057}$ & $\mathbf{0.024_{0.031}}$ & $\mathit{0.003_{0.001}}$ & $\mathit{0.003_{0.001}}$ & $0.009_{0.005}$ &	$\mathit{0.003_{0.001}}$\\ \cline{2-11}
%& $250$	& $0.483_{0.065}$ &	$\mathbf{0.011_{0.002}}$ &	$0.299_{0.071}$ &	$0.161_{0.058}$ &	$0.144_{0.163}$ & $0.076_{0.040}$ & $0.050_{0.018}$ &	$\mathbf{0.012_{0.010}}$\\ \cline{2-10}
& $300$	& $0.516_{0.068}$ &	$0.429_{0.068}$ &	$0.312_{0.061}$ &	$0.284_{0.224}$ & $\mathbf{0.237_{0.069}}$ & $0.034_{0.028}$ & $\mathit{0.021_{0.002}}$ & $0.022_{0.003}$ &	$0.022_{0.002}$\\ \hline\hline
\multirow{3}{*}{Kosarak}
& $50$ & $0.020_{0.044}$ &	$0.021_{0.053}$ &	$0.002_{0.005}$ &	$0.006_{0.028}$ & $\mathbf{0.001_{0.003}}$ & $0.002_{0.012}$ &	$\mathit{0.000_{0.001}}$ &	$\mathit{0.000_{0.001}}$  & $\mathit{0.000_{0.000}}$\\ \cline{2-11}
& $100$ & $0.140_{0.104}$ &	$0.036_{0.056}$ &	$\mathbf{0.018_{0.032}}$ &	$0.039_{0.082}$ & $0.025_{0.052}$ & $0.002_{0.018}$ & $\mathit{0.000_{0.001}}$ & $0.004_{0.003}$  &	$\mathit{0.000_{0.000}}$\\ \cline{2-11}
& $150$ & $0.640_{0.126}$ &	$0.042_{0.050}$ &	$\mathbf{0.008_{0.013}}$ &	$0.062_{0.109}$ & $0.015_{0.036}$ & $\mathit{0.001_{0.000}}$ & $0.003_{0.003}$ & $0.018_{0.007}$ &	$\mathit{0.001_{0.000}}$\\ \cline{2-11}
\multirow{2}{*}{$\epsilon=0.5$}
& $200$ & $0.869_{0.075}$ &	$0.430_{0.112}$ &	$0.085_{0.061}$ &	$0.077_{0.102}$ & $\mathbf{0.037_{0.045}}$ & $\mathit{0.004_{0.003}}$ & $\mathit{0.004_{0.002}}$  & $0.018_{0.007}$ &	$\mathit{0.004_{0.001}}$\\ \cline{2-11}
%& $250$ & $0.906_{0.070}$ &	$\mathbf{0.018_{0.003}}$ &	$0.707_{0.107}$ &	$0.349_{0.104}$ &	$0.207_{0.197}$ & $0.144_{0.092}$ & $0.458_{0.115}$ &	$\mathbf{0.019_{0.003}}$\\ \cline{2-10}
& $300$ & $0.936_{0.051}$ &	$0.845_{0.077}$ &	$0.628_{0.095}$ &	$0.423_{0.270}$ & $\mathbf{0.412_{0.123}}$ & $0.108_{0.086}$ & $\mathit{0.047_{0.004}}$ & $0.049_{0.003}$  & $0.048_{0.004}$\\ \hline\hline
\multirow{3}{*}{AOL}
& $50$ & $0.008_{0.010}$ & $0.005_{0.009}$ &	$0.005_{0.009}$ &	$0.006_{0.011}$ & $\mathbf{0.004_{0.005}}$ &	$0.001_{0.004}$ &  $0.002_{0.004}$ & $0.004_{0.006}$ & $\mathit{0.000_{0.000}}$\\\cline{2-11}
& $100$ & $0.017_{0.015}$ & $0.010_{0.009}$ &	$\mathbf{0.007_{0.007}}$ &	$0.022_{0.018}$ & $0.009_{0.009}$ & $\mathit{0.000_{0.001}}$ & $0.003_{0.005}$ & $0.020_{0.010}$ & $\mathit{0.000_{0.000}}$\\\cline{2-11}
& $150$ & $0.136_{0.029}$ & $0.013_{0.010}$ &	$0.008_{0.008}$ &	$0.020_{0.021}$ & $\mathbf{0.007_{0.007}}$ & 	$\mathit{0.000_{0.000}}$ & $0.001_{0.002}$ & $0.014_{0.009}$  &  $\mathit{0.000_{0.000}}$\\\cline{2-11}
\multirow{2}{*}{$\epsilon=0.5$}
& $200$ & $0.800_{0.032}$ & $0.016_{0.009}$ &	$\mathbf{0.008_{0.005}}$ &	$0.032_{0.031}$ & $\mathbf{0.008_{0.007}}$ & 	$\mathit{0.001_{0.000}}$ & $0.003_{0.004}$ & $0.023_{0.010}$  & $\mathit{0.001_{0.000}}$\\\cline{2-11}
%& $250$ & $0.967_{0.014}$ & $\mathbf{0.002_{0.001}}$ & $0.235_{0.027}$ &	$0.020_{0.010}$ &	$0.041_{0.036}$ & $0.012_{0.010}$ & $0.075_{0.016}$ &	$\mathbf{0.002_{0.001}}$\\\cline{2-10}
& $300$ & $0.988_{0.007}$ & $0.748_{0.031}$ &	$0.098_{0.017}$ &	$0.074_{0.070}$ & $\mathbf{0.018_{0.012}}$ & 	$\mathit{0.005_{0.002}}$ & $0.006_{0.003}$ & $0.036_{0.012
}$ & $\mathit{0.005_{0.001}}$\\\hline\hline
\multirow{3}{*}{Zipf}
& $50$ & $0.426_{0.142}$ & $0.034_{0.059}$ &	$0.011_{0.019}$ &	$0.022_{0.042}$ & $0.020_{0.043}$ &	$0.004_{0.032}$ &	$0.002_{0.003}$  & $0.009_{0.007}$ &	$\mathit{0.000_{0.000}}$ \\\cline{2-11}
& $100$ & $0.919_{0.061}$ & $0.808_{0.093}$ &	$0.571_{0.111}$ &	$0.353_{0.260}$ & $0.361_{0.138}$ & $0.090_{0.068}$ &	$0.035_{0.006}$  & $0.036_{0.006}$ &	$\mathit{0.033_{0.005}}$  \\\cline{2-11}
& $150$ & $0.935_{0.053}$ & $0.916_{0.052}$ &	$0.864_{0.072}$ &	$0.745_{0.224}$ & $0.784_{0.108}$ & $0.570_{0.143}$ &	$0.232_{0.126}$  & $0.114_{0.007}$ &	$\mathit{0.111_{0.007}}$ \\\cline{2-11}
\multirow{2}{*}{$\epsilon=0.5$}
& $200$ & $0.932_{0.054}$ & $0.919_{0.050}$ &	$0.896_{0.065}$ &	$0.848_{0.156}$ & $0.863_{0.077}$ & $0.734_{0.111}$ &	$0.435_{0.134}$  & $0.173_{0.024}$ &	$\mathit{0.170_{0.009}}$ \\\cline{2-11}
%& $250$ & $0.999_{0.002}$ & $\mathbf{0.571_{0.013}}$ & $0.998_{0.003}$ &	$0.995_{0.005}$ &	$0.978_{0.043}$ & $0.990_{0.008}$ & $0.996_{0.004}$ &	$\mathbf{0.977_{0.011}}$\\\cline{2-10}
& $300$ & $0.903_{0.067}$ & $0.912_{0.052}$ &	$0.899_{0.059}$ &	$0.832_{0.178}$ & $0.907_{0.058}$ & $0.767_{0.098}$ &	$0.484_{0.127}$  & $\mathit{0.247_{0.018}}$ &	$\mathit{0.247_{0.011}}$\\\hline\hline


\end{tabular}
\caption{Comparison of SVT-DPBook, SVT-S, SVT-ReTr and EM on selecting top-$c$ queries in terms of SER. For each row, the best SER value in the non-interactive setting is marked by italics and the best SER value in the interactive setting is marked by boldface.  Each cell gives the average value of SER with standard deviation. }\label{tab:method_comp_eps}
\end{table*}



